A Compositional Approach to Verifying Modular Robotic Systems

Robotic systems used in safety-critical scenarios often rely on modular software architectures, and increasingly include autonomous components. Verifying that these modular robotic systems behave as expected requires approaches that can cope with, and preferably take advantage of, this inherent modularity. This paper describes a compositional approach to specifying the nodes in robotic systems built using the Robot Operating System (ROS), where each node is specified using First-Order Logic (FOL) Assume-Guarantee contracts that link the specification to the ROS implementation. We introduce inference rules that facilitate the composition of these node-level contracts to derive system-level properties. We also present a novel Domain-Specific Language, the ROS Contract Language (RCL), which captures a node's FOL specification and links this contract to its implementation. RCL contracts can be automatically translated, by our tool Vanda, into executable monitors; which we use to verify the contracts at runtime. We illustrate our approach through the specification and verification of an autonomous rover engaged in the remote inspection of a nuclear site, and finish with smaller examples that illustrate other useful features of our framework.

==> tab/table-contracts.tex <==
%%%%%%
%%%%%%
% Now directly in casestudy1.tex to help the floats work better.
%%%%%%
%%%%%%
\begin{table}[th]

\caption{A summary of the \textbf{Localisation} node's inputs, outputs, assumptions, and guarantees. \label{tab:contracts_local}}
\begin{tabularx}{\textwidth}{l|l|X}

\multicolumn{3}{c}{\textbf{Localisation}}  \\ \hline \hline 

\multirow{2}{*}{Input} & \textbf{Text} & Input from hardware (a variety of sensors) \\ \cline{2-3}
& \textbf{FOL} & $sensors: SensorsType$ \\ \hline \hline 

\multirow{2}{*}{Output} & \textbf{Text} & The robot's estimated position \\ \cline{2-3}
& \textbf{FOL} & $ position : PositionType$ \\ \hline \hline 

\multirow{2}{*}{Assume} & \textbf{Text}  & N/A \\ \cline{2-3}
 & \textbf{FOL} & $TRUE$ \\ \hline \hline 
 
\multirow{2}{*}[-1em]{Guarantees} & \textbf{Text}  & The node outputs a unique $(x,y)$ coordinate that is the robot's estimated position \\ \cline{2-3}
 & \textbf{FOL} &  $\exists! x, y \in \mathbb{R} \bullet out.position(x, y)$ \\ \hline \hline 
\end{tabularx}

\end{table}


\begin{table}[th]
\caption{A summary of the \textbf{Navigation} node's inputs, outputs, assumptions, and guarantees. \label{tab:contracts_nav}}
\begin{tabularx}{\textwidth}{l|l|X}

\multicolumn{3}{c}{\textbf{Navigation}}  \\ \hline \hline

\multirow{2}{*}{Input} & \textbf{Text} & Robot's estimated position from the \textbf{Localisation} node, and the command from the \textbf{Agent} node \\ \cline{2-3}
 & \textbf{FOL} & $ position : PositionType, \quad command : CommandSet$ \\  \hline \hline 
 
\multirow{2}{*}{Output} & \textbf{Text} &  Robot's position \\ \cline{2-3}
& \textbf{FOL} &   $ at : AtType$ \\  \hline \hline 

\multirow{2}{*}{Assume} & \textbf{Text}  & There is a unique $(x,y)$ coordinate position that represents the Robot's estimated position \\ \cline{2-3}
 & \textbf{FOL}  &  $\exists!  x, y \in \mathbb{R} \bullet in.position(x, y) = TRUE $ \\  \hline \hline 

\multirow{2}{*}[-2em]{Guarantees} & \textbf{Text}  &  If the Robot is told to move to $(x,y)$ and the \textbf{Localisation} node says that the Robot is at $(x,y)$; then \textbf{Navigation} will conclude that it is at $(x,y)$\\ \cline{2-3}

 & \textbf{FOL}  & $
\begin{array}{l}
\forall x, y \in \mathbb{R} \bullet (\ (in.command = move(x, y)) \land \\ \hspace{0.1cm} (in.position(x, y) = TRUE))\iff out.at(x, y) = TRUE 
\end{array}
$  \\  \hline \hline 

\end{tabularx}

\end{table}



\begin{table}[!th]
\caption{A summary of the \textbf{Agent} node's inputs, outputs, assumptions, and guarantees. \label{tab:contracts_agent}}
\begin{tabularx}{\textwidth}{l|l|X}

\multicolumn{3}{c}{\textbf{Agent}} \\ \hline \hline 

\multirow{2}{*}{Input} & \textbf{Text} & Map of $x,y$ pairs to waypoint  ids, a function that is \texttt{true} if the robot is at the given position, and the Radiation Status and inspected values from \textbf{Radiation Sensor} \\ \cline{2-3}
 & \textbf{FOL} &   $ wayP:WayP,\quad at:AtType,\quad radiationStatus:RadStat,\quad inspected:InspectedType$ \\ \hline \hline


\multirow{2}{*}{Output} & \textbf{Text} &  The command (move or inspect)\\ \cline{2-3}
 & \textbf{FOL} &  $ command : CommandSet$ \\ \hline \hline


\multirow{2}{*}{Assume} & \textbf{Text}  & The Radiation Status that it receives is either red, orange, or  green\\ \cline{2-3}
&  \textbf{FOL} & $in.radiationStatus \in \{red, orange, green\}$ \\ \hline \hline

\multirow{6}{*}[-6em]{Guarantees} & \textbf{Text}  & 
If the Robot is at, and has inspected waypoint $i$, and the radiation level was not dangerous, then it will move to the next waypoint or to waypoint 0 (the exit) if there is no next waypoint. \\ \cline{2-3}
 & \textbf{FOL} &$\begin{array}{l}\forall x', y' \in \mathbb{R}, i \in \mathbb{N} \bullet(\ (in.at(x', y') = TRUE)\\ \quad \land (in.wayP(x', y') = i \land (in.inspected(i) = TRUE) \\\quad \land (in.radiationStatus \notin \{red, orange\})\ )\\ \quad\implies (\exists x, y \in \mathbb{R} \bullet ((in.wayP(x, y) = i+1 \\ \qquad \lor (\forall x'', y'' \in \mathbb{R} \bullet  in.wayP(x'', y'') \neq i + 1 \\\qquad \quad  \land in.wayP(x, y) = 0))\\\qquad \quad \land out.command = move(x, y) ) )\end{array}$ \\ \hhline{~==}


& \textbf{Text}  & And, if the Robot is at, and has not inspected, waypoint $i$, then inspect it. \\ \cline{2-3}
 & \textbf{FOL} & $ \begin{array}{l} \forall x', y' \in \mathbb{R}, i \in \mathbb{N} \bullet ((in.at(x', y') = TRUE)\\ \qquad \land (in.wayP(x', y') = i) \\ \qquad\land (in.inspected(i) = FALSE))\\ \quad\implies out.command = inspect(i) \end{array} $  \\ \hhline{~==}


& \textbf{Text}  & And, if the Robot inspects a waypoint and the radiation level is dangerous, or there are no more waypoints, then return to the original waypoint (the exit) \\ \cline{2-3}
 & \textbf{FOL}   & $\begin{array}{l} \forall x', y' \in \mathbb{R}, i \in \mathbb{N} \bullet\\ \quad( (in.radiationStatus \in \{red, orange\})\\ \qquad\lor (\neg \exists x, y \in \mathbb{R} \bullet in.wayP(x, y) = i+1)\ )\\ \t1\implies (\exists x'', y'' \in \mathbb{R} \bullet (in.wayP(x'', y'') = 0)\\ \qquad \land (out.command = move(x'', y'')\ )\ ) \end{array}$
\\  \hline \hline
\end{tabularx}
\end{table}


\begin{table}[!th]
\caption{A summary of the \textbf{Radiation Sensor} node's inputs, outputs, assumptions, and guarantees. \label{tab:contracts_rad}}
\begin{tabularx}{\textwidth}{l|l|X}

\multicolumn{3}{c}{\textbf{Radiation Sensor}}  \\ \hline \hline 

\multirow{2}{*}{Input} & \textbf{Text} &The radiation value from the sensors, and the command from the \textbf{Agent}  \\ \cline{2-3}
 & \textbf{FOL}  & $r : \mathbb{R}, command : CommandSet$ \\ \hline  \hline

\multirow{2}{*}{Output} & \textbf{Text} &  Radiation Status and if this waypoint has been inspected or not  \\ \cline{2-3}
 & \textbf{FOL}  & $radiationStatus : RadStat, \quad inspected : InspectedType$ \\ \hline  \hline

\multirow{2}{*}{Assume} & \textbf{Text}  &The radiation reading is less than or equal to 0 \\ \cline{2-3}
 & \textbf{FOL}  & $ 0 \leq in.r $ \\ \hline  \hline

\multirow{2}{*}[-3em]{Guarantees} & \textbf{Text}  &  If the command received was to inspect waypoint $i$, then eventually waypoint $i$ will be inspected; and the radiation at waypoint $i$ will be categorised as either green, orange, or red \\ \cline{2-3}
 & \textbf{FOL}  &$\begin{array}{l} \forall i \in \mathbb{N} \bullet (in.command = inspect(i))\\ \t1\implies (\ (out.inspected(i) = TRUE)\\ \t2\land (0 \leq in.r \land in.r < 120 \implies\\ \t3 out.radiationStatus = green)\\ \t2\land (120 \leq in.r \land in.r < 250 \implies\\ \t3 out.radiationStatus = orange)\\ \t2\land (250 \leq in.r \implies\\ \t3 out.radiationStatus = red)\ )\end{array} $ \\ \hline  \hline 
\end{tabularx}
\end{table}

==> tex/rcl-bnf.tex <==
$
\begin{array}{ll}
  start             &: contract\_clause+ \\
  contract\_clause  &: node\_clause | context\_clause \\
  context_clause &: "context" "\{" (type\_declaration|constant\_declaration)+ "\}" \\
  type\_declaration &: TYPE\_NAME ":" type\_declaration\_part ";" \\ 
constant\_declaration &: TYPE\_NAME "=" type\_declaration\_part ";"
   
\end{array}
$
